Constraining the Thin Disc Initial Mass Function using Galactic Classical Cepheids

Context: The Initial Mass Function (IMF) plays a crucial role on galaxy evolution and its implications on star formation theory make it a milestone for the next decade. It is in the intermediate and high mass ranges where the uncertainties of the IMF are larger. This is a major subject of debate and analysis both for Galactic and extragalactic science. Aims: Our goal is to constrain the IMF of the Galactic thin disc population using both Galactic Classical Cepheids and Tycho-2 data. Methods: For the first time the Besan\c{c}on Galaxy Model (BGM) has been used to characterise the Galactic population of the Classical Cepheids. We have modified the age configuration in the youngest populations of the BGM thin disc model to avoid artificial discontinuities in the age distribution of the simulated Cepheids. Three statistical methods, optimized for different mass ranges, have been developed and applied to search for the best IMF that fits the observations. This strategy allows us to quantify variations in the Star Formation History (SFH), the stellar density at Sun position and the thin disc radial scale length. A rigorous treatment of unresolved multiple stellar systems has been undertaken adopting a spatial resolution according to the catalogues used. Results: For intermediate masses, our study favours a composite field-star IMF slope of $\alpha=3.2$ for the local thin disc, excluding flatter values such as the Salpeter IMF ($\alpha=2.35$). Moreover, a constant Star Formation History is definitively excluded, the three statistical methods considered here show that it is inconsistent with the observational data. Conclusions: Using field stars and Galactic Classical Cepheids, we have found, above $1M_\odot$, an IMF steeper than the canonical stellar IMF of associations and young clusters. This result is consistent with the predictions of the Integrated Galactic IMF.

==> ZoomIMF2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,704){\makebox(0,0)[r]{\strut{} \Large-3}}%
      \put(946,1722){\makebox(0,0)[r]{\strut{}\Large-2.5}}%
      \put(946,2740){\makebox(0,0)[r]{\strut{}\Large-2}}%
      \put(946,3757){\makebox(0,0)[r]{\strut{}\Large-1.5}}%
      \put(946,4775){\makebox(0,0)[r]{\strut{}\Large-1}}%
      \put(1078,484){\makebox(0,0){\strut{} \Large 3}}%
      \put(2147,484){\makebox(0,0){\strut{}\Large 4}}%
      \put(3654,484){\makebox(0,0){\strut{}\Large 6}}%
      \put(4723,484){\makebox(0,0){\strut{}\Large 8}}%
      \put(5553,484){\makebox(0,0){\strut{} \Large10}}%
      \put(6803,484){\makebox(0,0){\strut{}\Large 14}}%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}\LARGE {log ($m^{-x}$)}}}}%
      \put(3940,154){\makebox(0,0){\strut{}\LARGE{Mass ($M_\odot$)}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5816,4541){\makebox(0,0)[r]{\strut{}\textbf{Salpeter IMF}}}%
      \csname LTb\endcsname%
      \put(5816,4278){\makebox(0,0)[r]{\strut{}\textbf{Kroupa-Haywood IMF}}}%
      \csname LTb\endcsname%
      \put(5816,4015){\makebox(0,0)[r]{\strut{}\textbf{Haywood-Robin IMF}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[]{ZoomIMF2}}%
    \gplfronttext
  \end{picture}%
\endgroup

